ComPar: Optimized Multi-Compiler for Automatic OpenMP S2S Parallelization

Parallelization schemes are essential in order to exploit the full benefits of multi-core architectures. In said architectures, the most comprehensive parallelization API is OpenMP. However, the introduction of correct and optimal OpenMP parallelization to applications is not always a simple task, due to common parallel management pitfalls, architecture heterogeneity and the current necessity for human expertise in order to comprehend many fine details and abstract correlations. To ease this process, many automatic parallelization compilers were created over the last decade. Harel et al. [2020] tested several source-to-source compilers and concluded that each has its advantages and disadvantages and no compiler is superior to all other compilers in all tests. This indicates that a fusion of the compilers' best outputs under the best hyper-parameters for the current hardware setups can yield greater speedups. To create such a fusion, one should execute a computationally intensive hyper-parameter sweep, in which the performance of each option is estimated and the best option is chosen. We created a novel parallelization source-to-source multi-compiler named ComPar, which uses code segmentation-and-fusion with hyper-parameters tuning to achieve the best parallel code possible without any human intervention while maintaining the program's validity. In this paper we present ComPar and analyze its results on NAS and PolyBench benchmarks. We conclude that although the resources ComPar requires to produce parallel code are greater than other source-to-source parallelization compilers - as it depends on the number of parameters the user wishes to consider, and their combinations - ComPar achieves superior performance overall compared to the serial code version and other tested parallelization compilers. ComPar is publicly available at: https://github.com/Scientific-Computing-Lab-NRCN/compar.

==> NAS.tex <==
% \par To further evaluate the compilers capabilities, we introduce a more practical test case. The Numerical Aerodynamics Simulations (NAS) Parallel Benchmarks \cite{bailey1991parallel}, developed and maintained by NASA, are a group of applications created to evaluate the performance of HPCs. The NAS Parallel Benchmarks include ten different benchmarks \cite{bailey2011parallel}. The benchmarks that were included to evaluate the compilers are Block Tri-diagonal solver (BT), Conjugate Gradient (CG), Embarrassingly Parallel (EP), Lower-Upper Gauss-Seidel solver (LU), Multi-Grid (MG), Scalar Penta-diagonal solver (SP) and Unstructured Adaptive mesh (UA). The benchmarks Fourier Transform (FT) and Integer Sort (IS) were excluded from this study due to the inability of AutoPar and Par4All to process them. Each of the benchmarks was processed by the three compilers and compiled using Intel(R) C Intel(R) 64 Compiler for applications running on Intel(R) 64, Version 18.0.1.163 Build 20171018 with a fixed class size defined by Class=C.\footnote[2]{Source code of relevant sections can be found at: $github.com/reemharel22/AutomaticParallelization\_NAS$} %The following figure \ref{fig:npb_serial_compare6a} presents the tools' speedup compared to the serial run of the benchmarks. 

  
% \subsection{NAS Results} \label{subsection51}
% \textbf{AutoPar} - Failed to gain any speedup in most of the benchmarks (BT, LU, MG, SP, EP). This can be explained by the insertion of OpenMP directives to computationally small loops, such as Listing \ref{autopar_ep} and the insertion of OpenMP directives in a nested loop manner, such as Listing \ref{autopar_sp}. 

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/autoPar_EP.c}
% \caption{AutoPar's directives on computationally small loops EP/ep.c.}
% \label{autopar_ep}
% \end{listing}
% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/autoPar_SP.c}
% \caption{AutoPar's directives on nested loop and low iterative loops SP/rhs.c.}
% \label{autopar_sp}
% \end{listing}

% \textbf{Par4All} - Unlike AutoPar, Par4All did not insert multiple directives in nested loops. However, Par4All did insert many of its directives on the innermost loops and on computationally small loops Listing \ref{p4a_lu_error}.

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/p4a_lu_error.c}
% \caption{Par4All's directives on computationally small and nested loops}
% \label{p4a_lu_error}
% \end{listing}

% \textbf{Cetus} - As mentioned above, Cetus ensures that the number of loop iterations is above ten thousand, combining this feature with the option to parallelize only the outermost-parallelizable loop in the loop nest explains the speedup gained in the CG, EP, LU, MG, SP benchmarks. Although this feature was found to be powerful in CG, EP, LU, MG, SP benchmarks, this is not the case in UA and BT benchmark, in which it was found to be insufficient in cases of a single loop such as Listing~\ref{cetus_bt}. UA and BT benchmark with the removed directives (single loops) speedup results are shown in table~\ref{fig:npb_man_serial6b}.

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/bt_cetus.c}
% \caption{Cetus directive in BT/x\_solve.c.}
% \label{cetus_bt}
% \end{listing}

% In order to show a more realistic scenario which involves the compilers' output and minimal human intervention. The unnecessary OpenMP directives, such as~\ref{autopar_sp}, created by the three compilers were \textbf{manually removed}. Table~\ref{fig:npb_serial_compare6a} presents the compilers' speedup compared to the serial run of the benchmarks whereas tables~\ref{fig:npb_man_serial6b} and~\ref{fig:npb_man_toolc} compare the compilers' performance after removing the unnecessary directives to the serial run and to the compilers' performance with those directives respectively. We can see that by removing the unnecessary OpenMP directive we gain speedup in most test-cases. These results imply that although the compilers results performed worse than the serial execution in some cases, we can still gain speedup with minimal human intervention by removing redundant directives. We can see that the compiler with the best results is Cetus. As one can see CG and EP benchmarks are the exceptions that disprove the rule, meaning without human intervention we still achieve the compilers' maximal speedup.

% \begin{figure}[H]

% \begin{subfigure}{\linewidth}
% \centering
% 	%1
%   \makebox[0pt]{%
%   \begin{tikzpicture}
%     \begin{axis}[
%   	width=16cm,
%   	height=4cm,
%       xmin=0,
%       ymajorgrids=true,
%       ylabel={Speedup},
%       enlarge x limits={abs=1.0cm},
%       ytick = {1,5,10,15,20},
%       ybar,
%       xtick=data,
%       xticklabels from table={Survey_Sheets/npb_speedup.csv}{Benchmark},
%       legend entries={
%       AutoPar,
%       Par4All,
%       Cetus,
%       }
%       ]
%       \addlegendimage{fill=mBlue}
%       \addlegendimage{fill=mRed}
%       \addlegendimage{fill=mYellow}
%      \addplot [fill=mBlue] table [x expr=\coordindex, y=AutoPar] {Survey_Sheets/npb_speedup.csv};
%       \addplot [fill=mRed] table [x expr=\coordindex, y=Par4All] {Survey_Sheets/npb_speedup.csv};
%       \addplot [fill=mYellow] table [x expr=\coordindex, y=Cetus] {Survey_Sheets/npb_speedup.csv};
%     \end{axis}
%   \end{tikzpicture}}
%   \caption{Speedup gained from the compilers alone on the tested benchmarks compared to serial execution.}
%   \label{fig:npb_serial_compare6a}

% \end{subfigure}

% \begin{subfigure}{\linewidth}
% \centering
% 	%2
%   \makebox[0pt]{%
%   \begin{tikzpicture}
%     \begin{axis}[
%   width=16cm,
%   height=4cm,
%       xmin=0,
%       ymajorgrids=true,
%       ylabel={Speedup},
%       enlarge x limits={abs=1.0cm},
%       ytick = {1,5,10,15,20},
%       ybar,
%       xtick=data,
%       xticklabels from table={Survey_Sheets/npb_speedup.csv}{Benchmark},
%       extra y tick labels={}
%       ]
%      \addplot [fill=mBlue] table [x expr=\coordindex, y=AutoPar] {Survey_Sheets/NPB_man_to_serial.csv};
%       \addplot [fill=mRed] table [x expr=\coordindex, y=Par4All] {Survey_Sheets/NPB_man_to_serial.csv};
%       \addplot [fill=mYellow] table [x expr=\coordindex, y=Cetus] {Survey_Sheets/NPB_man_to_serial.csv};
%     \end{axis}
%   \end{tikzpicture}}
%   \caption{Speedup gained from removing the unnecessary OpenMP directives compared to serial execution.}
%   \label{fig:npb_man_serial6b}
  
% \end{subfigure}

% \begin{subfigure}{\linewidth}
% \centering
% 	%3
%   \makebox[0pt]{%
%   \begin{tikzpicture}
%     \begin{axis}[
%   width=16cm,
%   height=4cm,
%       xmin=0,
%       ylabel={Speedup},
%       enlarge x limits={abs=1.0cm},
%       ytick = {1,10,20,30,40},
%       ymajorgrids=true,
%       ybar,
%       xtick=data,
%       xticklabels from table={Survey_Sheets/npb_speedup.csv}{Benchmark},
%       extra y tick labels={}
%       ]
%      \addplot [fill=mBlue] table [x expr=\coordindex, y=AutoPar] {Survey_Sheets/NPB_man_to_tool.csv};
%       \addplot [fill=mRed] table [x expr=\coordindex, y=Par4All] {Survey_Sheets/NPB_man_to_tool.csv};
%       \addplot [fill=mYellow] table [x expr=\coordindex, y=Cetus] {Survey_Sheets/NPB_man_to_tool.csv};
%     \end{axis}
%   \end{tikzpicture}}
%   \caption{Speedup gained from removing the unnecessary OpenMP directives compared to non-removal.}
%   \label{fig:npb_man_toolc}
  
% \end{subfigure}

% \caption{NAS benchmark results.}
% \label{fig:test}
% \end{figure}
% \subsection{OpenMP NAS Benchmark}
% In order to maximize the compilers' performance on the NAS benchmark - and by that to fully understand the parallelization compilers performances -  we introduced AutoPar, Par4All and Cetus to a parallel-suitable NAS benchmark~\cite{npbopenmp}, which was code-designed to achieve peak performances using OpenMP. The OpenMP NAS benchmarks tackle the same NAS serial benchmark physical and mathematical problems, with differences in the code structure, such as including OpenMP directives in the most suitable spots, pre-declaring global variables as shared or private if necessary, changing a loop to be more suitable for a reduction clause and so forth. The notion for testing the compilers on a code that was re-designed to be more suitable for shared-memory parallel run is obvious, as serial code not always enables achieving peak performances without the necessary adaptations. Therefore, the compilers should yield better performances on the NAS parallel-suitable codes. However, the performances results were almost identical to the results of the compilers with the serial benchmark. The following figure~\ref{fig:npb_openmp_tool6} compares the compilers' speedup on the OpenMP benchmark, after removing unnecessary OpenMP directives, as was discussed above in section~\ref{subsection51}, to the OpenMP benchmark ($\frac{Tool\ Runtime}{OpenMP\ Runtime}$).

% \begin{figure}[H]

% \centering
% 	%1
%   \makebox[0pt]{%
%   \begin{tikzpicture}
%     \begin{axis}[
%   	width=16.5cm,
%   	height=4cm,
%       ymajorgrids=true,
%       ylabel={ Speedup},
%       enlarge x limits={abs=1.0cm},
%       ybar,
%       xtick=data,
%       xticklabels from table={Survey_Sheets/npb_speedup.csv}{Benchmark},
%       log ticks with fixed point,
%       legend entries={
%       AutoPar,
%       Par4All,
%       Cetus,
%       }
%       ]
%       \addlegendimage{fill=mBlue}
%       \addlegendimage{fill=mRed}
%       \addlegendimage{fill=mYellow}
%      \addplot [fill=mBlue] table [x expr=\coordindex, y=AutoPar] {Survey_Sheets/NPB_omp_speedup.csv};
%       \addplot [fill=mRed] table [x expr=\coordindex, y=Par4All] {Survey_Sheets/NPB_omp_speedup.csv};
%       \addplot [fill=mYellow] table [x expr=\coordindex, y=Cetus] {Survey_Sheets/NPB_omp_speedup.csv};
%     \end{axis}
%   \end{tikzpicture}}
%   \caption{Speedup gained from removing the unnecessary OpenMP directives compared to the man-OpenMP code.}
%   \label{fig:npb_openmp_tool6}

% \end{figure}
% Although the code is different and more suitable for shared-memory parallelization, the compilers failed to take advantage of this parallelization adaptation in the code structure and did not gain any significant performance improvements. A comprehensive analysis of the causes to the gap between the original OpenMP code to the compiler's OpenMP code can be found in the next section.

% \subsection{The Gap between and Pitfalls of the Compilers} \label{pitfalls_of_tools}

% As known, the NAS OpenMP parallel benchmark contains many nested loops with an OpenMP directive on the outermost loop, which ensures minimal overhead from thread creation while maximizing the workload of each thread (for example, Listing~\ref{parallel_region_bt}). In some of these cases, the compilers failed to insert an OpenMP directive to the outermost loop or insert an OpenMP directive at all, as shown in Listing~\ref{cetus_bt}. The insertion of the directives into the inner loops resulted in smaller workloads for each thread, and therefore it increased the overhead penalty to the total runtime. The reasons for the gap between the original OpenMP parallelized code and the compilers’ OpenMP code and between the compilers themselves, can be summarized in the following points:

% \textbf{Internal logic of the code} - The OpenMP parallel benchmark contains code segments that are wrapped within a parallel region directive. Inside the parallel region, a team of threads is created once, and then is being executed on the same code segment. This is helpful in cases of consecutive loops that can be parallelized at once, thus minimizing the overhead caused by creating threads over and over again. Furthermore, this one-time-thread-creating parallel region allows the usage of the \textit{nowait} clause, an example of this is shown in Listing~\ref{parallel_region_mg}. Another example is when there is an assignment of individual work for each individual thread, as shown in Listing~\ref{parallel_region_ep}. Cases like Listing \ref{parallel_region_mg} and Listing \ref{parallel_region_ep} are hard to predict without knowing the internal logic of the code, which is the reason for the failure of the compilers to insert an OpenMP directive at all. The lack of the internal logic of the code might cause additional failures in producing OpenMP directives due to the difficulty of predicting or understanding the pattern of the code. For example, in Listing~\ref{logic_cg} the compilers can't predict the values of the array {\em rowstr} thus, the compilers must assume the worst case which is the values of the array contain overlapping range.

% \textbf{Array privatization} - Many of the OpenMP directives in the NAS OpenMP code include an array privatization. As mentioned, unlike Cetus, AutoPar and Par4All support only scalar variable privatization and not array privatization. Thus, AutoPar and Par4All failed to insert OpenMP directives into \textit{for}-loops that can be parallelized with the array privatization option while Cetus managed to do so successfully. Thanks to this feature, Cetus managed to produces the best results among the three compilers in most of the NAS benchmarks (Fig~\ref{fig:npb_serial_compare6a},~\ref{fig:npb_openmp_tool6}). The only exception test case is the CG test case, as the original CG OpenMP code did not include array privatization options.

% \textbf{Function calls} - Although Cetus and Par4All analyze function side effects automatically, in the NAS benchmark the analysis of function side effects were found to be insufficient. To analyze function side effects, the compiler needs the source code of the function and not the compiled form of the function at the compiler's processing stage. This is due to the fact that these compilers are source-to-source compilers. Even if the function's source code is provided to the compiler, in some cases it fails to analyze the side effect correctly, thus fails to insert an OpenMP directive entirely. 

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/bt_omp.c}
% \caption{OpenMP parallel region in BT/x\_solve.c.}
% \label{parallel_region_bt}
% \end{listing}

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/mg_omp.c}
% \caption{OpenMP parallel region in MG/mg.c.}
% \label{parallel_region_mg}
% \end{listing}

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/ep_omp.c}
% \caption{OpenMP parallel region in EP/ep.c.}
% \label{parallel_region_ep}
% \end{listing}

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/NAS_logic_cg.c}
% \caption{Array values defined in runtime in CG.}
% \label{logic_cg}
% \end{listing}

% \subsection{Overcoming the Pitfalls in The Limits of OpenMP 2.5}
% In order to overcome the pitfalls that were encountered by the compilers, and to minimize the gap between the original OpenMP code to the code produced by the compilers, we suggest several changes in the original OpenMP code that will help the compilers produce better results, i.e additional directives to additional loops, with minimal human intervention. However, there are some pitfalls that the presented compilers cannot overcome due to their inability to produce the directive such as defining a parallel region, the \textit{nowait} directive, array privatization option (although in specific cases loop transformations can be applied to eradicate the array or, if possible, by declaring the array inside the loop thus, implicitly declaring the array as private). It is worth noting that the changes we suggest can be used for the general case of these pitfalls and not only for the NAS benchmark.

% \textbf{Array privatization} - Although Cetus can produce an OpenMP directive with array privatization, it is still difficult to predict an array privatization case. Thus, if one has prior knowledge whether the loop can be parallelized with the array privatization option, the array can be declared inside the loop. Thus, implicitly declaring the array as a private array. By implicitly declaring the array as private, we also overcome Par4All's and AutoPar's pitfall - in which these compilers cannot produce an array privatization option at all. An example of producing an OpenMP directive by implicitly declaring an array as a private is shown in Listing~\ref{ap_bt}.

% \textbf{Function calls} - As mentioned, analyzing function side effects can be difficult and not all the compilers support this option. In order to overcome the function side effect pitfall, it might be helpful to 'inline' the function's source code to the loop itself. As seen in Listing~\ref{func_bt}, by inserting the function's source code Cetus managed to produce the correct OpenMP directive.

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/bt_x_solve_private_cetus.c}
% \caption{Implicitly declaring the array as private in BT/x\_solve.c.}
% \label{ap_bt}
% \end{listing}

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/bt_x_solve_function_cetus.c}
% \caption{Inserting binvcrhs source code to BT/x\_solve.c main loop.}
% \label{func_bt}
% \end{listing}

% In order to test the techniques discussed above, we apply the two techniques discussed above on three NAS benchmarks - BT, SP and MG.
% We targeted the three source codes in BT benchmark - \textit{x\_solve}, \textit{y\_solve}, \textit{z\_solve} due to their high execution time~\cite{prema2017identifying}. By applying the two techniques while maintaining the correctness of the code, Cetus managed to insert the correct and optimal directive in the new source codes while Par4All and AutoPar failed to produce the same result due to long analyzing time which resulted in the compilers failing in mid-process. A similar procedure was done for the two other benchmarks - SP and MG. In SP, Par4All and Cetus managed to insert the correct and optimal directive while AutoPar failed to produce the same directive. In MG applying the techniques did not help Cetus to produce better results, because the compiler already inserted the correct directives and avoided these pitfalls. Nonetheless, Par4All did overcome the pitfalls and managed to insert additional OpenMP directives while AutoPar failed to overcome the pitfalls.
% Figure \ref{fig:bt_new_54} presents the speedup of the compilers compared to the human-made OpenMP code. The bold bars represent the speedup gained after applying the discussed techniques, while the striped bars represent the speedup gained before applying these techniques (as in figure~\ref{fig:npb_openmp_tool6}). As one can notice, Cetus's BT execution time is shorter than the human's. This is due to the minimization of function calls in the new source code, which resulted in faster execution time.

% %TODO
% \begin{figure}[H]

% \centering
% 	%1
%   \makebox[0pt]{%
%   \begin{tikzpicture}
%     \begin{axis}[
%   	width=16cm,
%   	height=4cm,
%     ylabel={Speedup},
%     enlarge x limits={abs=1.0cm},
%     ytick = {0.2, 0.4, 0.6, 0.8, 1.0, 1.2},
%     legend style={at={(0.8, 0.6)}, anchor = east},
%     ybar,
%     ymajorgrids = true,
%     xtick={1,...,20},
%     xticklabels from table={Survey_Sheets/Cetus_BT_SP.csv}{Benchmark},
%     legend entries={
%         Par4All after,
%         Par4All before,
%         Cetus after,
%         Cetus before
%         }
%     ]
%      \addlegendimage{fill=mRed}
%      \addlegendimage{black, fill=mLightRed,postaction={ pattern=north east lines}}
%      \addlegendimage{fill=mYellow}%
%      \addlegendimage{black, fill=mLightYellow, postaction={ pattern=north east lines}}
      
%     \addplot [fill=mRed] table [x = index, y=Par4All] {Survey_Sheets/Cetus_BT_SP.csv};
    
%          \addplot[black, fill=mLightRed,postaction={ pattern=north east lines}] table [x = index,y=Par4AllA] {Survey_Sheets/Cetus_BT_SP.csv};
         
%     \addplot [fill=mYellow] table [ x = index, y=Cetus] {Survey_Sheets/Cetus_BT_SP.csv};
    
%     \addplot[black, fill=mLightYellow, postaction={ pattern=north east lines}] table [ x = index,y=CetusA] {Survey_Sheets/Cetus_BT_SP.csv};
    
%     \end{axis}
%   \end{tikzpicture}}
%   \caption{Speedup gained before and after applying the two techniques, compared to the human\-made OpenMP code.}
%   \label{fig:bt_new_54}

% \end{figure}
% %\subsection{Overcome Pitfalls in Limits of OpenMP 2.5}
% %XXX

% % \subsection{Overcome Pitfalls and Upgrade Code Performances in OpenMP 4.5} \label{NAS_omp4.5}
% % As discussed above, the different parallelization tools can identify complicated structures, such as the multi-loop structure, with some limitations (see \ref{pitfalls_of_tools}). Unfortunately, these tools can produce directives up to OpenMP 2.5, which means they can't produce \textit{SIMD} (Single Instruction Multiple Data) and \textit{target} constructs, nor use any of the \textit{thread affinity} features that were added in OpenMP 4.0 and enhanced in OpenMP 4.5.
% % As many current enterprise computers have an enlarge vector unit and hold heterogeneous configuration which contains CPUs alongside co-processors (such as Xeon-Phi) or accelerators (such as GPGPUs), the performance may be greatly improved - even by an order of magnitude - by manually inserting new OpenMP 4.5 directives in to the existing directives produced by the tools thus, using all of the hardware architecture benefits.

% % OpenMP 4.0 introduces the composite loop \textit{SIMD} construct \cite{van2017using}. A \textit{SIMD} instruction performs the same operation on multiple data simultaneously. Such an operation uses a special register that can hold multiple scalar elements. One of the advantages of \textit{SIMD} instruction is that it is almost as fast as its corresponding scalar instruction. Thus, the processor time can be potentially reduced by a factor of the register's width. The composite loop \textit{SIMD} construct first divides the loop iterations into chunks to be distributed between threads according to the clauses of the \textit{for} construct, and then these chunks may be translated to \textit{SIMD} loops according to the clauses of the \textit{SIMD} construct. This allows the programmer to easily identify code segments that can be converted into \textit{SIMD} loops and add the composite loop \textit{SIMD} construct to them. As current compilers do not successfully locate all of the optionally \textit{SIMD} code regions, this option can greatly increase code performances. 

% % Another OpenMP 4.5 directive that can be added is the \textit{target} construct. With the \textit{offload} directive the specified code can be easily offloaded to a co-processor or an accelerator in cases where the loop contains intensive operations, i.e. there are many iterations over the same code segments, thus making the tool produce parallel codes that are suited for heterogeneous architectures. This directive instructs to map the region of the \textit{target} construct to a device (such as GPGPU). This region will then be executed on the mapped device. Similar to the \textit{SIMD} directive, the programmer - as well as the parallelization tools - can detect the regions that will greatly benefit from this directive and add the \textit{target} construct to the directives that were already produced by the parallelization tools. However, executing on a device (co-processors or accelerator) and producing better performance than the CPU parallel execution is not guaranteed and requires fine-tuning adjustments to the scheme in order to fully benefit from these architectures. Additionally, mapping the variables from and to the device may lead to overhead thus, reducing the performances.
% % %Thus, the compiler can identify whether it is profitable to use this composite construct, for example by using the if-statements of the \textit{for} constructs provided by Cetus.

% % The idea that is presented here can be expanded even further by adding the OpenMP 4.5 directives automatically via the tools and is discussed in \ref{section7} for future work. Cetus inserts an if-statement with every OpenMP directive to minimize the overhead of thread creation. This technique can be broadened for the OpenMP 4.5 directives. For example, in order to insert a \textit{target} directive, the compiler can easily check if an argument fits the device memory-capacity and whether the overhead is not too big. One can extend the idea of the if-statement to check not only the number of iterations and operations but also memory usage, as known GPGPUs have less memory capacity than NUMA CPUs architectures. In addition, one can train the parallelization tools to identify code segments that can be converted to \textit{SIMD} loops and functions. Moreover, as will be discussed in \ref{section7}, the benefits and the new directives introduced in OpenMP 4.5 such as the thread-affinity, and placement, can be leveraged in order to find the directives that will produce the best performance.

% % In order to show XXX


==> Survey_Sheets/P4A_SP_MG.tex <==
Benchmark 

==> accelerators.tex <==
%   \par In this section we test Par4All's ability to transform C code to CUDA for GPUs. To better suite this study case, we slightly modified the previous matrix multiplication code see Listing \ref{mat_mul_gpu}.
% % * <matanru@post.bgu.ac.il> 2018-09-07T11:18:37.746Z:
% % 
% % > GUPs
% % GPUs
% % 
% % ^.
% \begin{itemize}  
% \item The new matrix is now allocated as a $N^2$ dimensional vector of integers instead of a $N$ dimensional vector of pointers to $N$ dimensional vectors of integers. 
% \item We replaced the dynamic parameter $n$ that holds the dimension of the matrix, with a static definition of $N$ known at compilation time (i.e \#define). \item We assume the matrix $B$ is transposed, which allows us to access it by row order, as is the access to the matrix $A$.

% \end{itemize}
% The above changes are required for Par4all to support the code transformation to CUDA and to enable better compiler optimization and memory management. Par4All's GPU accelerator support relies on an API called P4A\_ACCEL that provides an encapsulation of CUDA's API. Data-parallel loops are automatically transformed into CUDA kernels that are executed on GPUs. Ad hoc communications between the host memory and the GPU memory are generated to enable kernel execution. 
% We test the Par4All's CUDA output on a GPU against Par4Alls OpenMP output on a Xeon processor and a Xeon-Phi Co-processor. The following architectures were used to test this study case:

% \begin{itemize}
% \item \textit{GPU}: NVIDIA(R) Tesla(R) V100-PCIE-32GB.
% \item \textit{Xeon}: Intel(R) Xeon(R) CPU E5-2683 v4 2 process units with 16 cores each. 
% \item \textit{Xeon-Phi}: Intel(R) Xeon-Phi co-processor 5100 series (rev 11).
% \end{itemize}

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/mat_mul_gpu.c}
% \caption{Matrix multiplication code for the GPU case study}
% \label{mat_mul_gpu}
% \end{listing}


% The native compilation scheme is to firstly allocate the desired space on the GPU for each parallel loop nest, transfer the computation data to the GPU and finally launch the kernel and copy back the results from the GPU. Par4Alls output for GPU accelerators is shown in Listing \ref{mat_mul_gpu_p4a_gpu}. Par4All's code transformation to OpenMP remains the same as before see Listing \ref{p4a1}. The runtime and speedup results of these tests are shown in figure \ref{fig:figure61}. 

% The results below show a great differentiation between the different platforms. Although the GPU V100 is about seven-eight times stronger in terms of flop/s than the Xeon-Phi KNC, the KNC outperformed the V100. We can also see that since the automatic code parallelization cannot transform the code into a vectorized code, performances did not improve in comparison to the Xeon processor, and were even worsen over an increase of the matrix size. We can also notice that the Xeon processor's speedups stay steady as we increase the matrix size, but they are worsen in the Xeon-Phi in a semi-linear fashion. 

% Therefore, we conclude that though these source-to-source automatic parallelization compilers can achieve improvements to shared-memory platforms, they still cannot achieve the same kind of improvements to more complicated architectures such as accelerators or co-processors. This is mostly due to the lack of vectorization support by these compilers. These architectures are still required to be programmed in an \textit{ad-hoc} fashion to a specific problem by an expert programmer that can take many parameters into account as parallelization is being performed.

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C} {Survey_C_Files/mat_mul_p4a_gpu_1000.c}
% \caption{Matrix multiplication code for the GPU transformed by Par4All to Accel (CUDA)}
% \label{mat_mul_gpu_p4a_gpu}
% \end{listing}

%  \begin{figure}[H]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
  
%   \makebox[0pt]{%
%   \begin{tikzpicture}
%   \begin{semilogyaxis}[xmin=0,xmax=20000,ymin=0.001,ymax=200000,
% % 	\begin{axis}[
% 	ylabel={Execution Time (sec)},
%   	xlabel={Problem Size},
%   	height=6cm,
%   	width=7cm,
%     xtick={0,5000,10000,15000,20000},
%   	legend style={at={(0.48,0.99)},anchor=north east},
% %    extra y ticks={0.01,0.1,1,10,100},
% %    extra y tick labels={0.01,0.1,1,10,100},
%   legend entries={ Xeon, Xeon-Phi, GPU},
%     log ticks with fixed point
%   ]
% %    \addplot+[mark=o, color=black, solid] table [x=n,y=serial, col sep=comma] {Survey_Sheets/xeon_xphi_gpu_1d_matmul_-_run_times.csv};
%   \addplot+[mark=o, color=mBlue, solid] table [x=n,y=xeon, col sep=comma] {Survey_Sheets/xeon_xphi_gpu_1d_matmul_runtime.csv};
%   \addplot+[mark=o, color=mRed, solid] table [x=n,y=xphi, col sep=comma] {Survey_Sheets/xeon_xphi_gpu_1d_matmul_runtime.csv};
%   \addplot+[mark=o, color=mGreen, solid] table [x=n,y=gpu, col sep=comma] {Survey_Sheets/xeon_xphi_gpu_1d_matmul_runtime.csv};
% %    \end{axis}
%   \end{semilogyaxis} 
%   \end{tikzpicture}%
%   }
% %   \caption{execution time.}
%   \label{fig:scale11}
  
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering

%   \makebox[0pt]{%
%   \begin{tikzpicture}
%   \begin{axis}[xmin=0,xmax=21000,ymin=0,ymax=50,
%   height=6cm,
%   width=7cm,
%   ylabel={$$ Speedup },
%   xlabel={$$ Problem Size},
%   legend style={at={(0.98,0.99)},anchor=north east},
%   legend entries={ Xeon, Xeon-Phi, GPU}
%   ]
%   \addplot+[mark=o, color=mBlue, solid] table [x=n,y=xeon, col sep=comma] {Survey_Sheets/xeon_xphi_gpu_1d_matmul_speedup.csv};
%   \addplot+[mark=o, color=mRed, solid] table [x=n,y=xphi, col sep=comma] {Survey_Sheets/xeon_xphi_gpu_1d_matmul_speedup.csv};
%   \addplot+[mark=o, color=mGreen, solid] table [x=n,y=gpu, col sep=comma] {Survey_Sheets/xeon_xphi_gpu_1d_matmul_speedup.csv};
%   \end{axis} 
%   \end{tikzpicture}%
%   }
% %   \caption{speedup}
%   \label{fig:scale6a}
  
% \end{subfigure}
% \caption{Execution time and speedup comparison of Par4All output on Xeon and Xeon-Phi and GPU.}
% \label{fig:figure61}
% \end{figure}



==> comparison.tex <==
% In this section we present relevant definitions and criteria for the automatic parallelization compilers. We then compare the three compilers' outcomes, and point to the strengths and weaknesses of each compiler. Lastly, we present a runtime analysis of the parallelized code segments using different suitable hardware platforms. 

% \subsection{Criteria and Terminology}
% Relevant definitions and criteria for automatic parallelization compilers comparison include - but are not limited to - the following:

% \begin{itemize}

% \item Definitions:

% \begin{itemize}
% \item \textit{Pointer Aliasing}: Refers to the situation where the same memory location can be accessed using multiple different names (i.e pointers).

% \item \textit{Function Side Effect}: A function is said to have a side effect if it modifies addresses accessible outside its scope (i.e has any interaction with the rest of the program besides a return value).

% \item \textit{Array Privatization}: The act of declaring an array as a private variable in a parallel section.

% \item \textit{Loop Unrolling/Unwinding}: A loop transformation technique that attempts to optimize a program's execution speed at the expense of its binary size (excess code). An example to this optimization is shown in loop unroll test (Listing~\ref{loopunroll3serial})

% \item \textit{Reduction Clause}: An OpenMP clause that performs a reduction operator on a variable or an array.

% \end{itemize}

% \item Criteria:

% \begin{itemize}

% \item \textit{No-Aliasing Option}: A flag notifying the source-to-source compiler that there are no pointer aliasing in the code.

% \item \textit{Supported Language}: The set of programing languages on which the source-to-source compilers can operate.

% \item \textit{Array Reduction/Privatization}: How does the source-to-source compiler behave when a parallel directive can only be added with an array reduction clause or with an array declared as private? 

% \item \textit{Loop Unroll support}: Will the source-to-source compiler insert OpenMP directives to unrolled loops?


% \item \textit{Double Check Alias Dependence}: Does the source-to-source compiler check for dependencies other than pointer aliasing when the No-Aliasing option is turned on?


% \item \textit{Function call support}: Will the source-to-source compiler insert OpenMP directives to loops containing function calls with/without side effects?

% \item \textit{Nested Parallelism}: How does the source-to-source compiler behave on nested loops?


% \item \textit{OOP Compatible}: Does the source-to-source compiler support Object Oriented Programming languages and concepts?

% \end{itemize}

% \end{itemize}

% \subsection{Test-Cases}
% Several input source codes were made in order to show the differences between the output files generated by AutoPar, Par4All and Cetus, in order to both test and compare their capabilities. The basic source codes are Matrix Vector Multiplication and Matrix Multiplication~\cite{liangvectorization}, the latter's source code is presented below.
% Several variants of these problems were created, with each variant pointing to a different parallel shared memory management pitfall/obstacle for the purpose of the compilers' dependence analysis. The Matrix Vector Multiplication source code was not included due to the similarity in the OpenMP directives to the Matrix Multiplication source code. 


% \subsubsection{Nested Loops and Array Reduction}

% The test on Listing~\ref{serial1} contains a nested loop which implements a simple na\"ive Matrix Multiplication calculation. While Par4All (Listing~\ref{p4a1}) inserted OpenMP directive solely to the outermost loop, AutoPar (Listing~\ref{rose1}) was able to insert OpenMP directives to the two outermost loops, and Cetus (Listing~\ref{cetus1}) managed to insert OpenMP directives to all of the loops.
% %\captionsetup{labelfont=bf}
% % \captionof{listing}{Serial matrix multiplication code for the nested loop and reduction test-case}
% % \inputminted[breaklines = true, frame=lines, framesep=2mm,
%  %   baselinestretch=1.2, linenos]
%   % {C}{Survey_C_Files/mat_mul.c}
    
% \begin{listing}
% \inputminted[linenos,breaklines,xleftmargin=2em] {C}{Survey_C_Files/mat_mul.c}
%     \caption{Serial matrix multiplication code for the nested loop and reduction test-case.}
% \label{serial1}
% \end{listing}

% \begin{listing}
% \inputminted[linenos,breaklines,xleftmargin=2em]{C}{Survey_C_Files/mat_mul_p4a.c}
% \caption{Par4All output for the nested loop and reduction test-case.}
% \label{p4a1}
% \end{listing}

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C}{Survey_C_Files/mat_mul_rose.c}
% \caption{AutoPar output for the nested loop and reduction test-case.}
% \label{rose1}
% \end{listing}

% \begin{listing}[htb]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C}{Survey_C_Files/mat_mul_cetus.c}
% \caption{Cetus output for the nested loop and reduction test-case.}
% \label{cetus1}
% \end{listing}


% \subsubsection{Pointer Aliasing} \label{ssec:pointeraliasing}
% Listing~\ref{serial3} contains a pointer dereference test-case. This specific test-case caused Cetus to step into an internal error. When given the No-Aliasing option, AutoPar ignored all data dependencies and inserted an incorrect OpenMP directive to the innermost loop (Listing~\ref{rose3snippet}). Par4All did not manage to insert any OpenMP directive (even with the No-Aliasing option). However, if one changes the arrays from a static allocation to a dynamic one, i.e. a pointer to a matrix, Par4All will insert OpenMP directive when given the No-Aliasing option. Since Cetus and Par4All did not manage to insert the directives in both allocation modes, their codes are not presented.

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C}{Survey_C_Files/pointer_alias.c}
% \caption{Serial Code for the pointer dereference test-case.}
% \label{serial3}
% \end{listing}



% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C}{Survey_C_Files/pointer_alias_rose_snippet.c}
% \caption{The innermost loop of AutoPar's output for the pointer dereference test-case which is wrong.}
% \label{rose3snippet}
% \end{listing}

% \subsubsection{Loop Unrolling}
% In Listing~\ref{loopunroll3serial} we created a version of the original \textit{mat\_mul} function where in each iteration we changed four consequent array cells. AutoPar did not manage to insert any OpenMP directives, thus the code it has generated is not included. Par4All parallelized the outermost loop as before and managed to insert the correct directive, therefore the code generated by it is not presented for convenience reasons. As before, Cetus added OpenMP directives to all three loops. However, Cetus's output for the innermost loop (Listing~\ref{loopunroll3cetus}) is invalid since it contains a reduction clause for multiple array cells. This kind of reduction can not be compiled - as far as is known - by any compiler. On the runtime analysis section we omitted this invalid OpenMP directive.
% % * <matanru@post.bgu.ac.il> 2018-09-03T20:23:57.139Z:
% % 
% % > therefore the code generated by it is not presented for convenience reasons
% % 2 options: 1. If u changed the previous listing, you should include this one. 
% % 2. "convenience reasons" maybe switch to "space considerations"? When you say convenience reasons it should be convenient to the reader, not you (by not doing some "avoda sh-hora") 
% % 
% % - Also, maybe you meant that the listing in this section is wrong and not the previous one?
% % 
% % ^ <reemharel22@gmail.com> 2018-09-04T18:54:23.889Z:
% % 
% % I think we should remove the "for convience reasons" totaly. no need to explain. (GAL IDAN)
% %
% % ^.
% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C}{Survey_C_Files/loop_unroll3.c}
% \caption{Serial code for the loop unrolling test-case.		}
% \label{loopunroll3serial}
% \end{listing}

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C}{Survey_C_Files/loop_unroll3_cetus_snippet.c}
% \caption{The innermost loop of Cetus Output for the loop\_unrolling test-case.}
% \label{loopunroll3cetus}
% \end{listing}

% \subsubsection{Function Calls}
% On another test-case (Listing~\ref{serial2}), the innermost instruction was isolated into a function and replaced with a function call. Using this code arrangement, the matrix multiplication contains a function-call side effect. For this test-case, AutoPar couldn't parallelize the code without being fed with an annotation file. Cetus always assumes that function-calls will cause unexpected data manipulations and tries to evade these side-effects by avoiding any OpenMP directives. Meanwhile, Par4All handles function side-effects automatically and manages to insert the OpenMP directive to the outermost loop as before (Listing~\ref{par4all2}). Since AutoPar and Cetus did not insert OpenMP directives, their code is not presented. 

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C}{Survey_C_Files/function_calls2_short.c}
% \caption{Serial code for the function call test-case.}
% \label{serial2}
% \end{listing}

% \begin{listing}[H]
% \inputminted[linenos,breaklines,xleftmargin=2em]{C}{Survey_C_Files/function_calls2_p4a_snippet.c}
% \caption{Par4All output code for the function call test-case.}
% \label{par4all2}
% \end{listing}

% \subsection{Runtime Analysis}
% All the above-mentioned test-cases were compiled using Intel(R) C Intel(R) 64 Compiler for applications running on Intel(R) 64, Version 18.0.1.163 Build 20171018 using internal optimizations (i.e. -O3), and executed on a machine with two Intel(R) Xeon(R) CPU E5-2683 v4 process units with 16 cores each. We also executed these tests on an Intel(R) Xeon-Phi co-processor 5100 series (rev 11) in native mode. As far as we know, this kind of performance comparison of the of automatic parallelization compilers over Xeon-Phi co-processors is the first of its kind.
% \par Figure~\ref{fig:bargraph} compares the runtime of each output file generated by the three automatic parallelization compilers (AutoPar, Par4All, Cetus) and the original sequential source code. The functions (y-axis) are the code segments described in section~\ref{comparison4}.
% As seen in~\ref{fig:bargraph}, Par4All's overall performance is the best. This is because AutoPar and Cetus generated OpenMP directives in the inner-loops which creates a slight overhead. Cetus inserts a reduction clause on an array which also creates overhead. However, one can disable this feature and avoid inserting a reduction clause on arrays. AutoPar has the worst performance in \textit{\_loop\_unroll} because the compiler did not insert any OpenMP directives on loops that have been manually unrolled.
% %------------------------------------------------------------------ Bar Function comparison --------------------
% \begin{figure}[htb]
%   \centering
%   \makebox[0pt]{%
%   \begin{tikzpicture}
%     \begin{axis}[
%     width=14cm,
%     height=9cm,
%       xmin=0,
%       xlabel={$$ Function name},
%       title={Matrix dimension = 1,000x1,000x1,000},
%       ylabel={$$ Execution Time (sec)},
%       enlarge x limits={abs=1.0cm},
%       ybar,
%       xtick=data,
%       xticklabels from table={Survey_Sheets/dataForThousand.csv}{Function},
%       legend style={at={(0.65, 0.7)},anchor=south west},
%       legend entries={
%       Serial,
%       AutoPar,
%       Par4All,
%       Cetus
%       }
%       ]
%       \addlegendimage{fill=mGreen}
%       \addlegendimage{fill=mBlue}
%       \addlegendimage{fill=mRed}
%       \addlegendimage{fill=mYellow}
%       \addplot [fill=mGreen] table [x expr=\coordindex, y=Serial] {Survey_Sheets/dataForThousand.csv};
%       \addplot [fill=mBlue] table [x expr=\coordindex, y=AutoPar] {Survey_Sheets/dataForThousand.csv};
%       \addplot [fill=mRed] table [x expr=\coordindex, y=Par4All] {Survey_Sheets/dataForThousand.csv};
%       \addplot [fill=mYellow] table [x expr=\coordindex, y=Cetus] {Survey_Sheets/dataForThousand.csv};
%     \end{axis}
%   \end{tikzpicture}%
%   }
%   \caption{Functions execution time generated by the three compilers and serial execution.}
%   \label{fig:bargraph}
%   \end{figure}
% \par Figure~\ref{fig:scale1} compares the execution time of the parallelized and serial \textit{mat\_mul} test-case on Xeon processors (represented by circle markers on the figure) and Xeon-Phi co processors (represented by square markers on the figure) with the "-O3" option. As one may notice, the performance of the parallel execution on MIC architecture is worse than on x86\_64. Figure~\ref{fig:scale2} compares the speedup gained by the parallel execution on Xeon to the serial execution, the results scale well as they are on average above x25 while the optimum is x32 which is the number of threads.


% \begin{figure}[H]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
  
%   \makebox[0pt]{%
%   \begin{tikzpicture}
%   \begin{semilogyaxis}[xmin=0,xmax=5500,ymin=0.001,ymax=2000,
%   ylabel={$$ Execution Time (sec)},
%   xlabel={$$ Problem Size},
%   height=7cm,
%   width=7cm,
%   legend style={at={(0.55,0.02)},anchor=south west},
%   extra y ticks={0.01,0.1,1,10,100},
%   extra y tick labels={0.01,0.1,1,10,100},
%   legend entries={ Serial,
%   AutoPar,
%   Par4All,
%   Cetus,
%   Xeon,
%   Xeon-Phi
%   },
%   log ticks with fixed point
%   ]
%   \addlegendimage{no markers, mGreen, solid}
%   \addlegendimage{no markers, mBlue, solid}
%   \addlegendimage{no markers, mRed, solid}
%   \addlegendimage{no markers, mYellow, solid}
%   \addlegendimage{only marks, mark=o, solid}
%   \addlegendimage{only marks, mark=square, solid}
%   \addplot+[mark=o, color=mGreen, solid] table [x=Elements,y=Serial, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
%       \addplot+[mark=o, color=mBlue, solid] table [x=Elements,y=AutoPar, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
%       \addplot+[mark=o, color=mRed, solid] table [x=Elements,y=Par4All, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
%   \addplot+[mark=o, color=mYellow, solid] table [x=Elements,y=Cetus, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
%   \addplot+[mark=square, color=mBlue,dashed] table [x=Elements,y=AutoPar-XeonPhi, col sep=comma]{Survey_Sheets/dataforScaling_new.csv};
%          \addplot +[mark=square, color=mRed, dashed] table [x=Elements,y=Par4All-XeonPhi, col sep=comma]
%          {Survey_Sheets/dataforScaling_new.csv};
%          \addplot +[mark=square, color=mYellow, dashed] table [x=Elements,y=Cetus-XeonPhi, col sep=comma]
%          {Survey_Sheets/dataforScaling_new.csv};
%         \end{semilogyaxis} 
%   \end{tikzpicture}%
%   }
%   \caption{\textit{mat\_mul} execution time with different problem sizes in log-scale.}
%   \label{fig:scale1}
  
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering

%   \makebox[0pt]{%
%   \begin{tikzpicture}
%   \begin{axis}[xmin=0,xmax=5500,ymin=19,ymax=33,
%   height=7cm,
%   width=7cm,
%   ylabel={$$ Speedup },
%   xlabel={$$ Problem Size},
%   legend style={at={(0.35,0.02)},anchor=south west},
%   ytick = {20,22,24,26,28,30,32},
%     log ticks with fixed point,
%   legend entries={ 
%   AutoPar,
%   Par4All,
%   Cetus,
%   Optimal speedup
%   }
%   ]
%   \addlegendimage{no markers, mBlue, solid}
%   \addlegendimage{no markers, mRed, solid}
%   \addlegendimage{no markers, mYellow, solid}
%   \addlegendimage{no markers, mGreen, solid}
% 	\addplot+[mark=o, color=mBlue] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{AutoPar})}, col sep=comma] {Survey_Sheets/dataforScaling_new2.csv};
%       \addplot+[mark=o, color=mRed] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Par4All})}, col sep=comma] {Survey_Sheets/dataforScaling_new2.csv};
%   \addplot+[mark=o, color=mYellow] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Cetus})}, col sep=comma] {Survey_Sheets/dataforScaling_new2.csv};
%   \addplot[color=mGreen, domain=1:6000]{32};
%         \end{axis} 
%   \end{tikzpicture}%
%   }
%   \caption{\textit{mat\_mul} speedup with different problem sizes on Xeon}
%   \label{fig:scale2}
  
% \end{subfigure}
% \label{fig:test}
% \caption{Execution time and speedup comparison on Xeon and Xeon-Phi.}
% \end{figure}


% \paragraph{} The next figure~\ref{fig:Xeon_phi3} compares the speedup gain from executing the parallel source codes on a Xeon-Phi co-processor with the options "-O3" and "-O0". The reason for compiling with the "-O0" option is to demonstrate the source-to-source compilers' capabilities without any source-to-machine language compiler optimization. The difference between the "-O3" and "-O0" and other options, is further discussed in Chae Jubb paper~\cite{jubb2014loop}. The speedup gain with the option "-O3" is lower than the option "-O0", this is because the option "-O3" improves the execution time of the serial run more that it improves the parallel. The performance imbalance with the option "-O0" happens mainly because the overhead that is caused by creating many threads for each loop, outweighs the benefit we gain from the parallelization itself. Once the benefit of parallelizing the computation over many threads overcomes the overhead of the creation of a thread itself, we can see an increase in speedup (which occurs when N>3000). The results from figure~\ref{fig:scale1} and figure~\ref{fig:Xeon_phi3} imply that one should not solely rely on automatic parallelization compilers  when optimizing code for execution on Xeon-Phi. Previous work showed that efficient optimization for native MIC involves vectorization~\cite{jeffers2013intel}, tailoring of the perfect algorithm~\cite{lu2013optimizing} and careful instructions arrangement~\cite{heinecke2013design}. These optimizations are yet beyond the capabilities of the automatic parallelization compilers.


% \begin{figure}[htb]
% \centering
% 	\begin{tikzpicture}
%         \begin{axis}[
%             xmin=400,xmax=5100,
%             ymin=1,ymax=5,
%             height=6cm, width=12cm,
%             ylabel={$$ Speedup },
%             xlabel={$$ Problem Size},
%             legend style={at={(0.02,0.4)},anchor=south west},
%             ytick = {0,0.5,1,1.5,2,2.5,3,3.5,4,4.5,5},
%             % log ticks with fixed point,
%             legend entries={ 
%                 AutoPar O3,
%                 Par4All O3,
%                 Cetus O3,
%                 AutoPar O0,
%                 Par4All O0,
%                 Cetus O0,
%             }
%         ]
%         \addlegendimage{mLightBlue, mark=o, solid}
%         \addlegendimage{mLightRed, mark=triangle, solid}
%         \addlegendimage{mLightYellow, mark=square, solid}
%         \addlegendimage{mBlue,  mark=o, mark options={solid}, dashed}
%         \addlegendimage{mRed,  mark=triangle, mark options={solid}, dashed}
%         \addlegendimage{mYellow, mark=square, mark options={solid}, dashed}
%         \addplot+[color=mLightBlue, mark=o, solid] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{AutoPar-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
%         \addplot +[color=mLightRed, mark=triangle, solid] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Par4All-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
%         \addplot +[color=mLightYellow, mark=square, solid] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Cetus-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
%         \addplot+[color=mBlue, mark=o, mark options={solid}, dashed] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{AutoPar-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling.csv};
%         \addplot +[color=mRed, mark=triangle, mark options={solid}, dashed] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Par4All-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling.csv};
%         \addplot +[color=mYellow, mark=square, mark options={solid}, dashed] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Cetus-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling.csv};
%         \end{axis} 
%     \end{tikzpicture}%
%     \caption{\textit{mat\_mul} speedup on Intel Xeon-Phi compared to serial run (on Intel Xeon) with both -O3 and -O0 optimizations.}
% \label{fig:Xeon_phi3}
% \end{figure}


% % \begin{figure}[htb]
% % \centering
% % \begin{subfigure}{.5\textwidth}
% %   \centering
% %   \makebox[0pt]{%
% %   \begin{tikzpicture} 
% %   \begin{axis}[
% %   ylabel={$$ Speedup},
% %   xlabel={$$ Problem Size},
% %   legend style={at={(0.62,0.95)},anchor=north west},
% %   height=6cm,
% %   width=8cm
% %   ]        
% %   \addplot+[color=mBlue] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{AutoPar-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
% %   \addplot +[color=mRed] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Par4All-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
% %   \addplot +[color=mYellow] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Cetus-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling_new.csv};
% %   \addlegendentry{AutoPar};
% %   \addlegendentry{Par4All};
% %   \addlegendentry{Cetus};
% %     \end{axis}
% %   \end{tikzpicture}%
% %   }
% %   \caption{\textit{mat\_mul} speedup on Intel Xeon-Phi compared
% %   \\\hspace{\textwidth}
% %   to serial run (on Intel Xeon) with -O3.}
% %   \label{fig:Speedup_compare3}
  
% % \end{subfigure}%
% % \begin{subfigure}{.5\textwidth}
% %   \centering

% %   \makebox[0pt]{%
% %   \begin{tikzpicture} 
% %   \begin{axis}[
% %   ylabel={$$ Speedup},
% %   xlabel={$$ Problem Size},
% %   legend style={at={(0.05,0.95)},anchor=north west},
% %   height=6cm,
% %   width=8cm,
% %   ]        
% %   \addplot+[color=mBlue] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{AutoPar-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling.csv};
% %   \addplot +[color=mRed] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Par4All-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling.csv};
% %   \addplot +[color=mYellow] table [x=Elements,y expr={(\thisrow{Serial} / \thisrow{Cetus-XeonPhi})}, col sep=comma] {Survey_Sheets/dataforScaling.csv};
% %   \addlegendentry{AutoPar};
% %   \addlegendentry{Par4All};
% %   \addlegendentry{Cetus};
% %     \end{axis}
% %   \end{tikzpicture}%
% %   }
% %   \caption{\textit{mat\_mul} speedup on Intel Xeon-Phi compared
% %   \\\hspace{\textwidth}
% %   to serial run (on Intel Xeon) with -O0.}
% %   \label{fig:Speedup_compare4}

% % \end{subfigure}
% % \caption{Xeon-Phi speedup compared to serial run.}
% % \label{fig:Xeon_phi3}
% % \end{figure}
   
% %--------------------------------------------------------------
% To further understand the abilities of the compilers to maximize performance both on co-processors and processors, we present a Vector Matrix Multiplication test case. In this test we balanced the problem size with the number of repetitions to allow a fixed number of floating point operations in all tests. The focus of this test is to show the impact of memory usage over the L1, L2 and L3 cache sizes while maintaining the same workload operation-wise. The first execution size contains one matrix size of 240 elements which sums to 233kB, while our L1 cache is 64kB and L2 cache size is 256kB. The second execution size contains 3000 elements which sums up to 3604kB, while our L3 cache is 41mB. The third execution size contains 15180 elements which sums to 1gB. The results show in figure~\ref{fig:bargraph5} that the fastest execution time for Xeon is with 3000 elements. This is because the number of cache misses is the smallest (the problem's size is smaller than the L3 cache size). We can see that for 15180 elements test case the Xeon-Phi outperformed the Xeon, which can indicate that Xeon-Phi is beneficial for larger inputs.
% % * <matanru@post.bgu.ac.il> 2018-09-03T21:22:07.362Z:
% % 
% % >  is with 3000 elements this is because the number of cache misses is the smallest (the problem's size is smaller than the L3 cache size). We can see that for 15180 elements which can indicate that Xeon-Phi is beneficial for larger inputs.
% % -> "is with 3000 elements. This is because the number of cache misses is the smallest (the problem's size is smaller than the L3 cache size). We can see that for 15180 elements which can indicate that Xeon-Phi is beneficial for larger inputs."
% % 
% % - You forgot something in the second sentence
% % 
% % ^ <reemharel22@gmail.com> 2018-09-04T19:01:37.202Z:
% % 
% % done first thing.
% % added the forgot something
% % 
% % ^.
% % * <matanru@post.bgu.ac.il> 2018-09-03T21:18:46.612Z:
% % 
% % >  The first execution size contains one matrix size of 240 elements
% % -> " The first execution contains one matrix with 240 elements which sums to 233kB" (up to is "lechol ha yoter"). The other executions should be changed similarly
% % 
% % ^ <reemharel22@gmail.com> 2018-09-04T18:58:18.698Z:
% % 
% % done
% %
% % ^.
% %This test case 
% \begin{figure}[H]
%   \centering
%   \makebox[0pt]{%
% %   \begin{tikzpicture}
% %     \begin{semilogyaxis}[
% %   width=12cm,
% %   height=5cm,
% %      % xmin=0,
% %      % ymin=1,
% %      % ymax=200,
% %       xlabel={$$ Problem Size},
% %       title={Matrix Vector Multiplication scaling},
% %       extra y ticks={50,100,250,500,1000},
% %       extra y tick labels={50,100,250,500,1000},
% %       ylabel={$$ Execution Time (sec)},
% %       enlarge x limits={abs=1.5cm},
% %       ytick = {0,1,2.5,5,7.5,10,12.5,15,17.5,2000},
% %       xtick=data,
% %       xticklabels from table={Survey_Sheets/vector_matrix.csv}{Elements},
% %       ybar,
% % 	legend entries={AutoPar,
% %    Par4All,
% %    Cetus,
% %    Xeon,
% %    Xeon-Phi
% %        },   log ticks with fixed point
% %       ]
% %     \addlegendimage{fill=mBlue}
% %    \addlegendimage{fill=mRed}
% %    \addlegendimage{fill=mYellow}
% %     %\addlegendimage{aquamarine, solid}
% %   %     \addlegendimage{dark red, solid}
% %    \addlegendimage{fill=cyan}
% %    \addlegendimage{fill=darkgray}
% % \addlegendimage{fill=lime}
% % %  \addlegendimage{only marks, mark=o, solid}
% % %  \addlegendimage{only marks, mark=square, solid}
% %       \addplot[fill=blue] table [x expr=\coordindex,y=AutoPar] {Survey_Sheets/vector_matrix.csv};
% %        \addplot[fill=black] table [x expr=\coordindex,y=Par4All] {Survey_Sheets/vector_matrix.csv};
% %    \addplot[fill=green] table [x expr=\coordindex,y=Cetus] {Survey_Sheets/vector_matrix.csv};
% %    \addplot[fill=cyan] table [x expr=\coordindex,y=XP-AutoPar]{Survey_Sheets/vector_matrix.csv};
% %          \addplot [fill=darkgray] table [x expr=\coordindex,y=XP-Par4All] {Survey_Sheets/vector_matrix.csv};
% %         \addplot [fill=lime] table [x expr=\coordindex,y=XP-Cetus] {Survey_Sheets/vector_matrix.csv};
% %     \end{semilogyaxis}
% %   \end{tikzpicture}%

% \begin{tikzpicture}
%         \begin{semilogyaxis}[
%             width=12cm,
%             height=5cm,
%             % xmin=0,
%             % ymin=1,
%             ymax=5000,
%             xlabel={$$ Problem Size},
%             title={Matrix Vector Multiplication scaling},
% %             extra y ticks={50,100,250,500,1000},
% %             extra y tick labels={50,100,250,500,1000},
%             ylabel={$$ Execution Time (sec)},
%             enlarge x limits={abs=1.5cm},
%             ytick = {0,50,100,250,500,1000,2000},
%             xtick=data,
%             xticklabels from table={Survey_Sheets/vector_matrix.csv}{Elements},
%             ybar,
%     	    legend entries={
%     	        AutoPar,
%                 Par4All,
%                 Cetus,
% %                 Xeon,
% %                 Xeon-Phi
%                 AutoPar Xeon-Phi,
%                 Par4All Xeon-Phi,
%                 Cetus Xeon-Phi
%             },
%             log ticks with fixed point
%         ]
%         \addlegendimage{fill=mBlue}
%         \addlegendimage{fill=mRed}
%         \addlegendimage{fill=mYellow}
% %         \addlegendimage{fill=white}
% %         \addlegendimage{black, fill=white, postaction={ pattern=north east lines}}
%         \addlegendimage{black, fill=mLightBlue, postaction={ pattern=north east lines}}
%         \addlegendimage{black, fill=mLightRed, postaction={ pattern=north east lines}}
%         \addlegendimage{black, fill=mLightYellow, postaction={ pattern=north east lines}}
%         \addplot[fill=mBlue] table [x expr=\coordindex,y=AutoPar] {Survey_Sheets/vector_matrix.csv};
%         \addplot[fill=mRed] table [x expr=\coordindex,y=Par4All] {Survey_Sheets/vector_matrix.csv};
%         \addplot[fill=mYellow] table [x expr=\coordindex,y=Cetus] {Survey_Sheets/vector_matrix.csv};
%         \addplot[black, fill=mLightBlue, postaction={ pattern=north east lines}] table [x expr=\coordindex,y=XP-AutoPar]{Survey_Sheets/vector_matrix.csv};
%         \addplot [black, fill=mLightRed, postaction={ pattern=north east lines}] table [x expr=\coordindex,y=XP-Par4All] {Survey_Sheets/vector_matrix.csv};
%         \addplot[black, fill=mLightYellow, postaction={ pattern=north east lines}] table [x expr=\coordindex,y=XP-Cetus] {Survey_Sheets/vector_matrix.csv};
%         \end{semilogyaxis}
%     \end{tikzpicture}%
%   }
%   \caption{Functions execution time generated by the three compilers and serial execution.}
%   \label{fig:bargraph5}
%   \end{figure}

